Experience Report: Developing the Servo Web Browser Engine using Rust

All modern web browsers - Internet Explorer, Firefox, Chrome, Opera, and Safari - have a core rendering engine written in C++. This language choice was made because it affords the systems programmer complete control of the underlying hardware features and memory in use, and it provides a transparent compilation model. Servo is a project started at Mozilla Research to build a new web browser engine that preserves the capabilities of these other browser engines but also both takes advantage of the recent trends in parallel hardware and is more memory-safe. We use a new language, Rust, that provides us a similar level of control of the underlying system to C++ but which builds on many concepts familiar to the functional programming community, forming a novelty - a useful, safe systems programming language. In this paper, we show how a language with an affine type system, regions, and many syntactic features familiar to functional language programmers can be successfully used to build state-of-the-art systems software. We also outline several pitfalls encountered along the way and describe some potential areas for future research.

==> lstlang-bomil.tex <==
\lstdefinelanguage{BOMIL}{%
  morekeywords={%
    addr, alloc, and, any, apply, bool, byte, case, ccall, cont, define, do, double,%
    end, enum, extern, false, float, fun, host_vproc, if, in, inline, int, let, long, module,%
    noreturn, promote, pure, return, short, tag, throw, true, typedef, unwrap, use_rw,%
    vec128, void, vproc, vpload, vpstore, wrap,%
  },%
  keywordsprefix=@,
  % otherkeywords={(,),[,],\{,\},\,,:,...,_,|,=,=>,->,\#,:>},
  sensitive,%
  morecomment=[n]{(*}{*)},%
  morestring=[d]",%
}[keywords,comments,strings]%


==> lstlang-manticore.tex <==
\lstdefinelanguage{Manticore}[]{SML}{%
  morekeywords={by,otherwise,pcase,pval,spawn,to},
  % otherkeywords={(|,|),[|,|],(,),[,],\{,\},\,,:,...,_,|,=,=>,->,\#,:>},
  otherkeywords={(|,|),[|,|],?,\&},
}[keywords,comments,strings]%


==> lstlang-pml.tex <==
\lstdefinelanguage{PML}[]{SML}{%
  morekeywords={by,otherwise,pcase,pval,spawn,to},
  % otherkeywords={(|,|),[|,|],(,),[,],\{,\},\,,:,...,_,|,=,=>,->,\#,:>},
  otherkeywords={(|,|),[|,|],?,\&},
}[keywords,comments,strings]%


==> lstlang-sml.tex <==
\lstdefinelanguage{SML}{%
  morekeywords={%
    abstype, and, andalso, as, case, datatype, do, else, end, eqtype, exception,%
    fn, fun, functor, handle, if, in, include, infix, infixr, let, local, nonfix,%
    of, op, open, orelse, raise, rec, sharing, sig, signature, struct, structure,%
    then, type, val, where, while, with, withtype,%
  },%
  % otherkeywords={(,),[,],\{,\},\,,:,...,_,|,=,=>,->,\#,:>},
  sensitive,%
  morecomment=[n]{(*}{*)},%
  morestring=[d]",%
}[keywords,comments,strings]%


==> slide-defs.tex <==
% slide-defs.tex
%
% common definitions for talks.
%
% define \TalkDate and \TalkTitle for footers
%

% for a 1024x768 screen, we have a 1.0:0.75 ratio.
\setlength{\textwidth}{9.3in}
\setlength{\textheight}{7.2in}
\addtolength{\leftmargin}{-0.15in}
\addtolength{\topmargin}{-0.7in}

\usepackage{color}
\usepackage{graphicx}
\usepackage{times}

%
% the following magic makes the tt font in math mode be the same as the
% normal tt font (i.e., Courier)
%
\SetMathAlphabet{\mathtt}{normal}{OT1}{pcr}{n}{n}
\SetMathAlphabet{\mathtt}{bold}{OT1}{pcr}{bx}{n}

\definecolor{Red}{rgb}{0.8,0.0,0.0}
\definecolor{Green}{rgb}{0.0,0.4,0.0}
\definecolor{Blue}{rgb}{0.0,0.0,0.9}
\definecolor{Purple}{rgb}{0.5,0.0,0.4}
\definecolor{Black}{rgb}{0.0,0.0,0.0}
\definecolor{Yellow}{rgb}{1.0,1.0, 0.25}
\definecolor{Cyan}{rgb}{0.25,1.0, 1.0}
\newcommand{\blue}[1]{\color{Blue}{#1}}
\newcommand{\red}[1]{\color{Red}{#1}}
\newcommand{\green}[1]{\color{Green}{#1}}
\newcommand{\purple}[1]{\color{Purple}{#1}}
\newcommand{\textblue}[1]{\textcolor{Blue}{#1}}
\newcommand{\textred}[1]{\textcolor{Red}{#1}}
\newcommand{\textgreen}[1]{\textcolor{Green}{#1}}
\newcommand{\textpurple}[1]{\textcolor{Purple}{#1}}
\newcommand{\textblack}[1]{\textcolor{Black}{#1}}

\newcommand{\mobycodecolor}{\color{Purple}}
\newcommand{\punctcolor}{\color{Blue}}
\newcommand{\kwcolor}{\color{Blue}}
\newcommand{\bolcodecolor}{\color{Green}}
\newcommand{\ccodecolor}{\color{Purple}}
%\newcommand{\highlightC}[1]{\textred{#1}}
\newcommand{\highlightC}[1]{\colorbox{Yellow}{#1}}
\newcommand{\highlightCC}[1]{\colorbox{Cyan}{#1}}

\newcommand{\BlueBullet}{\textcolor{Blue}{\ensuremath{\bullet}}}
\newcommand{\RedBullet}{\textcolor{Red}{\ensuremath{\bullet}}}
\newcommand{\GreenBullet}{\textcolor{Green}{\ensuremath{\bullet}}}

\newcommand{\EM}[1]{\emph{\textred{#1}}}

\raggedright
\pagestyle{empty}

\newcommand{\HEAD}[1]{
  \noindent{\large\bf{}#1}\\[-1ex]
  \textblue{\hrulefill}\\[1em]}
\newcommand{\CONTINUE}[1]{
  \noindent{\bf{}#1 {\it{}(continued ...)}}\\[-1ex]
   \textblue{\hrulefill}\\[1em]}
\newcommand{\CHEAD}[1]{{\makebox[\textwidth]{\large\bf{}#1}\\[1em]}}
\newcommand{\FOOT}{%
  \vfill\textblue{\hrulefill}\\ %
  \tiny{
    \mbox{\rule[-.5ex]{0em}{3ex}} %
    \TalkDate  \hfill \TalkTitle \hfill \arabic{slide}}%
}

\newenvironment{FIGURE}{%
  \begin{center}\small}{%
  \end{center}}

% code
\newcommand{\tkw}[1]{\text{\kw{#1}}}
\newcommand{\tcd}[1]{\text{\cd{#1}}}
 
